Streaming Video Analytics On The Edge With Asynchronous Cloud Support

Emerging Internet of Things (IoT) and mobile computing applications are expected to support latency-sensitive deep neural network (DNN) workloads. To realize this vision, the Internet is evolving towards an edge-computing architecture, where computing infrastructure is located closer to the end device to help achieve low latency. However, edge computing may have limited resources compared to cloud environments and thus, cannot run large DNN models that often have high accuracy. In this work, we develop REACT, a framework that leverages cloud resources to execute large DNN models with higher accuracy to improve the accuracy of models running on edge devices. To do so, we propose a novel edge-cloud fusion algorithm that fuses edge and cloud predictions, achieving low latency and high accuracy. We extensively evaluate our approach and show that our approach can significantly improve the accuracy compared to baseline approaches. We focus specifically on object detection in videos (applicable in many video analytics scenarios) and show that the fused edge-cloud predictions can outperform the accuracy of edge-only and cloud-only scenarios by as much as 50%. We also show that REACT can achieve good performance across tradeoff points by choosing a wide range of system parameters to satisfy use-case specific constraints, such as limited network bandwidth or GPU cycles.

==> introduction_old.tex <==

Unmanned Aerial Vehicles (UAVs) are unique mobile sensing platforms for monitoring our natural and human-made environments from a vantage point. Unlike the conventional manned aircrafts, UAVs can fly at lower altitudes to yield better data collection at high-resolution in a cost-effective manner without the need to put human lives in harm's way --- especially in inaccessible terrains or hazardous conditions. UAVs have shown initial adoption in several domains such as agriculture~\cite{puri2017agriculture,vasisht2017farmbeats}, transportation~\cite{flammini2016railway}, renewables~\cite{ismail2019autonomous,wang2017automatic}, construction~\cite{hubbard2015feasibility}, disease control~\cite{amenyo2014medizdroids}, ecological conservation~\cite{koh2012dawn,schiffman2014drones}, surveillance~\cite{bolkcom2008homeland}, search and rescue~\cite{silvagni2017multipurpose} etc. Thus, commercial drone use for infrastructure monitoring grew at an annual rate of 19\% from 2016 to 2020 and is expected to grow at a tremendous pace in the next few years ~\cite{sachs2017drones}.   

Although promising, most of these applications deploy UAVs as ``dumb'' video recording devices, with most of the data analysis happening in the cloud. The availability of cloud resources allows running bigger deep learning models for the inference that provide higher accuracy. However, due to bandwidth restrictions, real-time execution on the cloud can endure significant latency that often gives way to offline processing of the inference pipeline. An alternate approach to overcome these limitations is to have the processing of the drone's video data using onboard compute, which enables real-time video stream processing. The advent of powerful edge devices --- such as Google's Coral TPU and Nvidia's Jetson series devices --- allows executing increasingly complex tasks. However, the lower latency on these compute platforms is aided not only by removing network delays from the cloud but also by running tiny machine learning models enforced by resource constraints at the edge. This reduction in compute operations for inference is often associated with an undesirable trade-off of having lower accuracy. 

Such a trade-off arises in several other use cases with real-time constraints such as building AR/MR application for mobile devices~\cite{zhang2018jaguar}, tracking suspicious activity through security cameras ~\cite{xu2018real}, triggering driver alerts using vehicle dash camera~\cite{nambi2018farsight}, etc. For all these scenarios, including UAV video processing, we need to run a computer vision pipeline that includes various tasks --- i.e., frame re-sizing, frame sampling, etc. along with running an object detection algorithm on the selected frames. The best configurations for a given pipeline depend on the various factors specific to the use case under consideration. We will discuss these in more detail in section~\ref{sec:background}.

In this paper, we explore the possibility of using the resources at both the edge and the cloud to get the best of both worlds, i.e., real-time execution with improved accuracy. Specifically, we present a system to leverage cloud resources capable of running larger models with higher accuracy to ``correct'' the past output of the edge devices and cascade these results for current predictions. We accomplish this by not executing tasks on the cloud synchronous with the edge execution, thereby eliminating the impact of network delays and inference times from the cloud to impact the latency observed by users of edge devices. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{graphs/illustrations/DroneImageProcess_new.pdf}
    \caption{}
    \label{fig:motivating_example}
\end{figure}

Intuitively, we illustrate our approach using the Figure~\ref{fig:motivating_example}, which shows a flood-affected area near the banks of the river taken from a UAV at two different times. Better human detection can help guide the UAV to track them. The frame at $T=0$ is sent to the cloud. The object detection model at the edge has lower accuracy, as indicated by several humans not being identified. The edge receives these annotations from the cloud models at $T=k$. Even though the scene has changed, there are a few objects that are common across the two frames. Thus, the edge --- by following the camera and object movements --- can selectively take the annotations that overlap over the two images to come up with better detections. Thus, asynchronous execution of object detection on past frames can still help in improving the accuracy of current frames seen at the edge. 

In this paper, we present our work that builds on the above intuition to create a system by improving the performance of object detections at the edge with minimum overheads. In particular, we make the following contributions - 
\begin{enumerate}
    \item \textbf{Cloud-side Pipeline:}
    \item \textbf{Edge-side Pipeline:} Use of other sensors such as IMU
    \item \textbf{Multi-objective formulation:}
    \item \textbf{Extensive evaluation:} We evaluate our system on multiple datasets.  
    \item \textbf{Wide-ranging applicability:} Further, we show that our work can open several exciting avenues that can be exploited by system developers to provide improved performance to the owners of edge devices. 
\end{enumerate}



%Further, real-time processing allows tremendous agility to 

%But issues of lower accuracy models.


%the data generated of computations happening offline there are many situations where it is advantageous to have on-board intelligence on the drone itself so that the sensor stream can be processed locally. 

%Qualities needed real-timeness, hardware constraints, lower latency, limited connectivity, higher accuracy, etc.

%Over the past few years, there has been a significant increase in the deployment of IoT sensors led by falling sensor costs and improvements in network connectivity. An interesting way of monitoring our environments is to equip 




%First, drones enable monitoring hazardous situations from a vantage point without the need to put human lives in harm's way --- for example, the inaccessible terrain or toxic environments resulting from natural or human-made disasters.

%Thus, BVLOS flights allow greater \textbf{safety} to drone operators. Second, BVLOS flights are \textbf{cost-effective} as drones can collect more data with fewer deployments and landing steps. In VLOS flights, the ground crew needs to move to keep pace with the drone. Finally, unlike the human-crewed aircrafts, drones can fly at lower altitudes and can yield \textbf{better data collection} at high-resolution. 


%With a growing need of reducing latency and taking decisions locally, there is a trend towards having a more popular edge devices are increasingly popular.  

%Increasingly these cyber-physical systems are enabled with edge devices that not only sense but also have compute capability. 


%Over the years, the processing capability of edge devices has improved significantly. This improvement has been across the board, i.e.,  mobile devices. This increase in performance has enabled a plethora of use cases, especially running deep learning inference.   

%Improving the performance of inference on edge is pivotal in many cyber-physical systems. 
 %Still for complex tasks we may not get real-time inference. 

%Sequential tasks

%Other considerations - network, power consumption

%Contributions


%Increasingly, we interface with natural and human-made environments rich with sensors. The proliferation of sensors is primarily lead by ava--- typically embedded devices --- allows massive data collection and processing is carried out either in offline cloud servers or in edge devices equipped with compute capability.  

%have also enabled are now have compute capability, which makes real-time analysis possible from sensor data possible.  


%Several closed-loop cyber-physical environments necessitate real-time analysis of IoT data closer to the edge. The advent of powerful edge devices allows executing increasingly complex tasks for several use cases at interactive speeds compared to cloud-enabled solutions. However, the lower latency of edge devices is aided not only by removing network delays from the cloud but also by running tiny machine learning models. This reduction in compute operations for inference is often associated with an undesirable trade-off of having lower accuracy. In this work, we leverage cloud resources capable of running larger models with higher accuracy to ``correct'' the past output of the edge devices and cascade these results for current predictions, thereby getting the best of both worlds. We believe that our work can open several exciting avenues that can be exploited by system developers to provide improved performance to the users. In this paper, we show the feasibility of our approach for two tasks with sequential data, i.e., object tracking. Moreover, this client-server system can be optimized to handle changing network conditions, server load, and client-side bandwidth limitations. 


%Increasingly, we interface with environments rich with sensors. The promise of such cyber-physical systems is making everything smart. 

==> table.tex <==
% \begin{table}[]
% \begin{tabular}{|l|l|l|}
% \hline
% Method    & D^2-City & Au-Air \\ \hline
% CenterNet &         &         \\ \hline
% FRCNN     &         &         \\ \hline
% YOLO      & 34.18   &         \\ \hline
% TinyYOLO  & 27.94   & 14.29   \\ \hline
% SSD       & ??      & ??      \\ \hline
% \end{tabular}
% \end{table}

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
                                             &           & \multicolumn{9}{c|}{AU-AIR}                                                           \\ \hline
                                             & Model     & Human  & Car & Truck & Van & Motorbike  & Bicycle          & Bus      & Trailer & mAP \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Cloud}} & CenterNet & 8.3   & 28.2 & 38.6 & 37.2 & 6.2 &  6.7 &  15.7  & 10.0        & 18.9    \\ \cline{2-11} 
\multicolumn{1}{|c|}{}                       & FRCNN     &        &     &       &     &            &                  &          &         &     \\ \cline{2-11} 
\multicolumn{1}{|c|}{}                       & YOLO      &        &     &       &     &            &                  &          &         &     \\ \hline
\multirow{2}{*}{Edge}                        & TinyYOLO  & 3.06   &32.40& 34.06 &30.35&   0.0      &        4.21      & 10.25    & 0.0     & 14.29     \\ \cline{2-11} 
                                             & MV2-SSD   &        &     &       &     &            &                  &          &         &     \\ \hline

                                             &           & \multicolumn{9}{c|}{D$^2$-City}                                                       \\ \hline

                                             & Model     & Person & Car   & Truck & Van   & Motorcycle-Tricycle & Bicycle & Bus   & Forklift-Block & mAP                 \\ \hline
\multirow{3}{*}{Cloud}                       & CenterNet & 38.4   & 74.8  & 46.0  & 38.0  & 27.0                & 26.2    & 60.7  & 4.2            &  39.4               \\ \hline \cline{2-11} 
                                             & FRCNN     & 34.0   & 60.3  & 42.9  & 30.1  & 28.7                 & 21.8     & 51.5  & 5.2            &  34.3                     \\ \hline \cline{2-11} 
                                             & YOLO      & 25.4   & 66.5  & 36.6 & 20.4 & 18.3                  & 16.3    & 52.3  & 2.3            & 29.8               \\ \hline
\multirow{2}{*}{Edge}                        & TinyYOLO  & 5.3    & 44.8  & 19.5  & 17.6  & 4.8                 & 4.1     & 27.2  & 0.1            & 15.4               \\ \cline{2-11} 
                                             & MV2-SSD   & 5.4    & 45.6  & 13.4  & 14.2  & 1.8                 & 3.0     & 28.4  & 0.0            & 14.0                \\ \hline
\end{tabular}%
    }
\caption{\hl{*******add it to appendix}Accuracy of Models \hl{cloud potential edge vs cloud}: for different models perform differently classes. Scene might change and so performance may change }
\label{tab:model_accuracy}
\end{table*}


